The effect of phased recurrent units in the classification of multiple catalogs of astronomical lightcurves

In the new era of very large telescopes, where data is crucial to expand scientific knowledge, we have witnessed many deep learning applications for the automatic classification of lightcurves. Recurrent neural networks (RNNs) are one of the models used for these applications, and the LSTM unit stands out for being an excellent choice for the representation of long time series. In general, RNNs assume observations at discrete times, which may not suit the irregular sampling of lightcurves. A traditional technique to address irregular sequences consists of adding the sampling time to the network's input, but this is not guaranteed to capture sampling irregularities during training. Alternatively, the Phased LSTM unit has been created to address this problem by updating its state using the sampling times explicitly. In this work, we study the effectiveness of the LSTM and Phased LSTM based architectures for the classification of astronomical lightcurves. We use seven catalogs containing periodic and nonperiodic astronomical objects. Our findings show that LSTM outperformed PLSTM on 6/7 datasets. However, the combination of both units enhances the results in all datasets.

==> Tables/data_table_old.tex <==
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{c|c|c|c|c}
        Label & Quantity & Max obs & Min obs & Mean obs\\ \hline\hline
        Be & 128 & 1641 & 273 & 921.26 \\
        CEPH & 101 & 1246 & 622 & 1170.61 \\
        EB & 255 & 1251 & 515 & 1167.73 \\
        LPV & 365 & 1246 & 64 & 1089.15 \\
        MOA & 582 & 1810 & 19 & 735.89 \\
        QSO & 59 & 1591 & 54 & 682.54 \\
        RRL & 610 & 1249 & 350 & 1101.08 \\ \hline
        \textbf{Total}  &  \textbf{2100}  \\ 
    \end{tabular}
    \caption{MACHO dataset composition}
    \label{tab:macho_dataset}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{c|c|c|c|c}
        Label & Quantity & Max obs & Min obs & Mean obs\\ \hline\hline
        Beta\_Persei & 291 & 653 & 79 & 292.61 \\ \hline
        Delta\_Scuti & 70 & 595 & 85 & 259.40 \\ \hline
        RR\_Lyrae\_FM & 2234 & 1150 & 33 & 264.94 \\ \hline
        RR\_Lyrae\_FO & 749 & 1004 & 38 & 280.69 \\ \hline
        W\_Ursae\_Maj & 1860 & 682 & 30 & 264.33 \\ \hline
        \textbf{Total}  &  \textbf{5204}  \\ \hline
    \end{tabular}
    \caption{LINEAR dataset composition}
    \label{tab:linear_dataset}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{c|c|c|c|c}
        Label & Quantity & Max obs & Min obs & Mean obs\\ \hline\hline
        Beta Persei  &  349  &  1072  &  137  &  488.1 \\ \hline
        Classical Cepheid  &  130  &  947  &  56  &  508.4 \\ \hline
        RR Lyrae FM  &  798  &  1600  &  77  &  410.5 \\ \hline
        Semireg PV  &  184  &  1729  &  152  &  504.9 \\ \hline
        W Ursae Maj  &  1639  &  1745  &  7  &  491.7 \\ \hline
        \textbf{Total}  &  \textbf{3100}  \\ \hline
    \end{tabular}
    \caption{ASAS dataset composition}
    \label{tab:asas_dataset}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{c|c|c|c|c}
        Label & Quantity & Max obs & Min obs & Mean obs\\ \hline\hline
        EC & 6862 & 2000 & 301 & 1235.13 \\ \hline
        ED & 21503 & 1530 & 300 & 540.02 \\ \hline
        ESD & 9475 & 2000 & 300 & 818.97 \\ \hline
        Mira & 6090 & 1987 & 300 & 795.62 \\ \hline
        OSARG & 234932 & 2000 & 300 & 828.56 \\ \hline
        RRab & 25943 & 1999 & 300 & 656.51 \\ \hline
        RRc & 7990 & 1998 & 300 & 683.89 \\ \hline
        SRV & 34835 & 2000 & 300 & 790.56 \\ \hline
        cep & 7836 & 1988 & 300 & 753.29 \\ \hline
        dsct & 2822 & 1961 & 307 & 636.30 \\ \hline
        std & 34815 & 421 & 300 & 346.83 \\ \hline
        \textbf{Total}  &  \textbf{393103}  \\ \hline
    \end{tabular}
    \caption{OGLE dataset composition}
    \label{tab:ogle_dataset}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{c|c|c|c|c}
    Label & Quantity & Max obs & Min obs & Mean obs\\ \hline\hline
Blazkho & 243 & 451 & 83 & 226.02 \\ \hline
CEPII & 277 & 526 & 52 & 250.85 \\ \hline
DSC & 147 & 350 & 78 & 232.16 \\ \hline
EA & 300 & 509 & 58 & 280.79 \\ \hline
EA\_UP & 153 & 508 & 104 & 291.90 \\ \hline
ELL & 142 & 526 & 105 & 336.19 \\ \hline
EW & 300 & 508 & 59 & 257.04 \\ \hline
HADS & 242 & 519 & 88 & 320.86 \\ \hline
LPV & 300 & 497 & 50 & 222.30 \\ \hline
Misc & 298 & 339 & 48 & 214.64 \\ \hline
RRab & 300 & 465 & 67 & 203.37 \\ \hline
RRc & 300 & 504 & 66 & 266.78 \\ \hline
RRd & 300 & 501 & 78 & 273.04 \\ \hline
RS\_CVn & 300 & 533 & 66 & 307.78 \\ \hline
Rotational Var & 300 & 352 & 67 & 241.71 \\ \hline
Transient & 300 & 458 & 1 & 133.66 \\ \hline
beta\_Lyrae & 279 & 538 & 116 & 316.50 \\ \hline
\textbf{Total}  &  \textbf{4481}  \\ \hline
    \end{tabular}
    \caption{CSS dataset composition}
    \label{tab:cata_dataset}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{c|c|c|c|c}
    Label & Quantity & Max obs & Min obs & Mean obs\\ \hline\hline
    CEP & 1884 & 161 & 20 & 72.25 \\ \hline
    DSCT\_SXPHE & 1098 & 157 & 20 & 34.92 \\ \hline
    Mira & 1396 & 165 & 20 & 86.90 \\ \hline
    NC & 2237 & 197 & 20 & 83.72 \\ \hline
    NonVar & 32795 & 139 & 20 & 84.78 \\ \hline
    OSARG & 53890 & 171 & 20 & 86.51 \\ \hline
    RRab & 16412 & 173 & 20 & 35.80 \\ \hline
    RRc & 3831 & 182 & 20 & 34.90 \\ \hline
    SRV & 8605 & 165 & 20 & 88.00 \\ \hline
    \textbf{Total}  &  \textbf{122148}  \\ \hline
    \end{tabular}
    \caption{WISE dataset composition}
    \label{tab:wise_dataset}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{c|c|c|c|c}
    Label & Quantity & Max obs & Min obs & Mean obs\\ \hline\hline
    CEP & 6484 & 232 & 11 & 33.30 \\ \hline
    DSCT\_SXPHE & 8579 & 233 & 11 & 24.73 \\ \hline
    MIRA\_SR & 150215 & 236 & 12 & 25.97 \\ \hline
    RRAB & 153392 & 242 & 11 & 23.51 \\ \hline
    RRC & 32206 & 241 & 11 & 26.76 \\ \hline
    RRD & 829 & 233 & 11 & 28.42 \\ \hline
    T2CEP & 1736 & 189 & 11 & 29.07 \\ \hline
    \textbf{Total}  &  \textbf{353441}  \\ \hline
    \end{tabular}
    \caption{GAIA dataset composition}
    \label{tab:gaia_dataset}
\end{table}


% \begin{table}
%     \centering
%     \scriptsize
%     \begin{tabular}{c|c|c|c|c}
%     Label & Quantity & Max obs & Min obs & Mean obs\\ \hline\hline
%     AGN & 548 & 446 & 12 & 159.33 \\ \hline
%     Blazar & 231 & 564 & 13 & 198.92 \\ \hline
%     CV & 792 & 523 & 11 & 143.79 \\ \hline
%     Flare & 184 & 524 & 11 & 224.97 \\ \hline
%     HPM & 294 & 394 & 11 & 78.77 \\ \hline
%     Non-Transient & 56871 & 5888 & 11 & 141.07 \\ \hline
%     SN & 1127 & 412 & 11 & 71.12 \\ \hline
%     Unknown & 61 & 409 & 11 & 68.62 \\ \hline
%     \textbf{Total}  &  \textbf{60108}  \\ \hline
%     \end{tabular}
%     \caption{GAIA dataset composition}
%     \label{tab:gaia_dataset}
% \end{table}



% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c}
%         Dataset & SNR mean & SNR std \\ \hline\hline
%         GAIA & 11868.69 & 9461.94 \\ \hline
%         OGLE & 2368.48 & 877.63 \\ \hline
%         LINEAR & 697.39 & 529.38 \\ \hline
%         MACHO & 337.96 & 590.11 \\ \hline
%         WISE & 308.77 & 118.65 \\ \hline
%         ASAS & 308.31 & 97.91 \\ \hline
%         CSS & 208.83 & 54.58 \\ \hline
%     \end{tabular}
%     \caption{Signal to Noise Ratio moments for each survey.}
%     \label{tab:SNR}
% \end{table}
% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c}
%         Dataset & Cadence mean & Cadence std \\ \hline\hline
%         CSS & 29.03 & 112.91 \\ \hline
%         GAIA & 23.69 & 36.01 \\ \hline
%         LINEAR & 7.65 & 30.71 \\ \hline
%         ASAS & 5.53 & 18.78 \\ \hline
%         OGLE & 3.69 & 13.35 \\ \hline
%         WISE & 2.65 & 20.27 \\ \hline
%         MACHO & 2.58 & 7.79 \\ \hline
%     \end{tabular}
%     \caption{Mean and standard deviation for each dataset cadence}
%     \label{tab:cadences}
% \end{table}
